Profiling Gas Consumption in Solidity Smart Contracts

Nowadays, more and more applications are developed for running on a distributed ledger technology, namely dApps. The business logic of dApps is usually implemented within smart contracts developed through Solidity, a programming language for writing smart contracts on different blockchain platforms, including the popular Ethereum. In Ethereum, the smart contracts run on the machines of miners and the gas corresponds to the execution fee compensating such computing resources. However, the deployment and execution costs of a smart contract depend on the implementation choices done by developers. Unappropriated design choices could lead to higher gas consumption than necessary. In this paper, we (i) identify a set of 19 Solidity code smells affecting the deployment and transaction costs of a smart contract, and (ii) assess the relevance of such smells through a survey involving 34 participants. On top of these smells, we propose GasMet, a suite of metrics for statically evaluating the code quality of a smart contract from the gas consumption perspective. An experiment involving 2,186 smart contracts demonstrates that the proposed metrics have direct associations with deployment costs. The metrics in our suite can be used for more easily identifying source code segments that need optimizations.

==> Implementation.tex <==
\textcolor{red}{ANDREA: Per spiegare metriche e tool farei un'unica sezione (magari possiamo chiamare la sezione 5: "The GasMet suite and tool" senza bisogno di suddividerla in sottosezioni (tipo implementation, using gasMet, etc.). Nel descrivere il tool oltre a dire che \'e basato su una grammitica antlr dovreste dare qualche dettaglio in pi\'u. Un po' come fatto con iSCREAM dovremmo descrivere come avviene il parsing ed il calcolo delle metriche. }

\major{For helping smart contract developers more easily identifying likely gas-inefficient code portions in smart contracts written in Solidity, we implemented the GasMet tool.}
%We empirically characterize gas cost savings based on a representative dataset of Ethereum smart contracts written in Solidity. For this, we implemented the Gasmet tool, as an open source tool for helping researchers and practitioners more easily identifying gas-inefficient code portions in smart contracts, and conducted the first empirical study on the prevalence of gas-inefficient code in the deployed smart contracts. 
%\major {\subsection{Implementation}}
\major{
GasMet is a prototype Java tool able to parse Solidity smart contracts and automatically compute the metrics in the GasMet suite. In particular, for properly parsing smart contracts, %written through both older and newer versions of the Solidity language, 
the tool leverages a generated parser based on a modified version of an existing \texttt{antlr4}  grammar\footnote{\url{https://github.com/solidityj/solidity-antlr4}}. %\textcolor{red}{La grammatica è valida solo per la versione 0.4 di Solidity}. 
%Cost smell information and description is stored in a mysql database.
The Widfly server was used to deploy the tool.

%The tool was implemented using the java language, using an existing grammar.

}

%\major {\subsection{Using GasMet}}
\major{
The tool either provides a graphical user interface (GUI) or can be used from the command line. The instructions for running the GUI or using it from the command line are provided in our replication package. Once selected a Solidity smart contract to analyze, the tool's GUI presents two frames (see Figure \ref{fig:metricResult}),. The left frame reports a table containing the results of the GasMet metrics computation on the selected smart contract. More specifically, the aforementioned table encompasses the following information about each metric: acronym, extended name, description, computed value, and lines involved in the computation. In the right frame, the source code of the smart contract under analysis is shown. The lines involved in the computation of the different GasMet metrics are highlighted in red to allow developers and researchers more easily identifying the code portions that could likely require improvements. A developer interested in saving the gas required for the deployment of her smart contract could analyze the smart contract through the GasMet tool and apply improvements to achieve better values for the computed metrics.    



%The tool can be used in two ways: through a graphical interface or through command line. By using the graphical interface, it is possible to choose a smart contract to analyze, upload it and show the results.
%In the results shown on the screen there are two tables. In the first column are present the results of the metrics (name of the metric, description and row in which this metric has been calculated), instead in the second column the source code of the uploaded file is shown with the number of rows and rows in which the metrics highlighted in red have been calculated.
%Instead, using the command-line tool, after running the jar, it is necessary to insert the .sol file to analyze. After this operation, the results of the metrics for the specific analyzed file will be shown on the screen. (Further details are available in the replication package.)

}


%\major {\subsection{Example / Scenario}}

 \begin{figure*}[h!]
    \centering
    \includegraphics[width=0.90\textwidth]{images/metricResult.png}
    \caption{Running example metric}
    \label{fig:metricResult}
\end{figure*}
